Towards gain tuning for numerical KKL observers

This paper presents a first step towards tuning observers for general nonlinear systems. Relying on recent results around Kazantzis-Kravaris/Luenberger (KKL) observers, we propose an empirical criterion to guide the calibration of the observer, by trading off transient performance and sensitivity to measurement noise. We parametrize the gain matrix and evaluate this criterion over a family of observers for different parameter values. We then use neural networks to learn the mapping between the observer and the nonlinear system, and present a novel method to sample the state-space efficiently for nonlinear regression. We illustrate the merits of this approach in numerical simulations.

==> sections/5_towards_optimization.tex <==
\section{Towards joint optimization}
\label{sec:towards_optimization}

In the previous sections, we approximate the transformation $\Tinv$ (and $\T$ if needed) using supervised learning.
However, it could be beneficial to directly optimize $D$ jointly with the transformations $\Tparam$ and $\Tinvparam$ instead of tuning it a posteriori. This is not possible with supervised learning, since $D$ needs to be fixed to build the dataset $(x_i, z_i)$. To address this shortcoming, we propose another approach based on an unsupervised learning framework: autoencoders.

\subsection{Autoencoders}
\label{subsec:learning_transformations_jointly}

Finding latent representations of the available data is an active research area in machine learning. In this regard, most state-of-the-art techniques are based on autoencoders (AE).
These consist in two neural networks that are trained jointly to learn the projection of an input into a latent space and back into the original space. 
Their aim is usually to find a meaningful, lower-dimensional representation of the data, in order to ease downstream tasks such as analysis or classification~\citep{Tschannen_recent_advances_autoencoder_representation_learning}, or to generate synthetic samples~\citep{Doersch_tutorial_variational_autoencoders}.

Autoencoders can also embed an input into a space with some known structure. This structure can be probabilistic, as often for variational AEs~\citep{kingma_auto-encoding_2013}, but can also derive from some known behavior of the latent space.
For example, in~\citet{Lusch_deeplearning_universal_linear_embeddings_nonlin_dyns}, the authors propose an AE framework to learn a linear approximation of general nonlinear systems relying on the Koopman operator. The AE model approximates the projection from the original coordinates to the corresponding Koopman coordinates, in which the system behaves linearly, and back. The linear but infinite-dimensional Koopman operator that acts in these coordinates is approximated jointly with the AE, by enforcing that the latent state follows linear dynamics driven by this operator.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=8.4cm]{figures/ae_schematics.pdf} % The printed column width is 8.4 cm.
		\setlength{\belowcaptionskip}{-8pt}
        \setlength{\abovecaptionskip}{-2pt}
		\caption{Structure of the autoencoder. The AE learns $\T$, $\Tinv$ by minimizing the loss~\eqref{eq:optimization_jointly} made up of the PDE~\eqref{eq:pdeT} and the reconstruction error between $\hat{x}$ and $x$.}
		\label{fig:kkl_ae}
	\end{center}
\end{figure}

Similarly to~\citet{Lusch_deeplearning_universal_linear_embeddings_nonlin_dyns,Nadri_autoencoder_KKL_discrete_time}, we propose to learn $\T$ and $\Tinv$ as a deterministic AE such that the latent variable $z$ verifies~\eqref{eq:dynz}. As presented in Sec.~\ref{sec:KKL_observers} and contrarily to standard AE models, under the assumptions at hand, the existence of suitable $\T$ and $\Tinv$ is guaranteed with fixed dimension $d_z$ and fixed structure of the latent space.

The AE is trained on $N$ samples $x_i$ obtained from a chosen sampling method; there is no need to sample $z$, which eases the data generation process.
It consists of two neural networks: an encoder and a decoder. The encoder $\Tparam$ maps the input to the latent state $z = \Tparam(x)$, and the decoder $\Tinvparam$ maps it back to a reconstruction of the input $\hat{x} = \Tinvparam(z)$. During training, the weights $\param$ and $\invparam$ are updated to minimize the following cost function:
\begin{align}
	\label{eq:optimization_jointly}
	L_{AE}(\param) = & \frac{1}{2} \sum_{x_i} \lambda \normltwo{ x_i - \Tinvparam(\Tparam(x_i)) }^2 + 
	\notag
	\\ 
	& \normltwo{ \frac{\partial \Tparam}{\partial x} (x_i) f(x_i) - D\Tparam(x_i) - F h(x_i)  }^2 .
\end{align}
The cost function is made up of two parts. First, the reconstruction loss, i.e., the mean squared error between $x_i$ and $\Tinvparam(\Tparam(x_i))$, enforces $x \approx \Tinvparam(\Tparam(x))$. 
Second, the partial differential equation (PDE)~\eqref{eq:pdeT} on $\T$ is enforced on the grid of $x_i$. Therefore, minimizing~\eqref{eq:optimization_jointly} boils down to approximating an invertible solution of~\eqref{eq:pdeT}.
The loss terms are weighted by the scalar $\lambda$. 
The architecture of the AE model is illustrated in Fig.~\ref{fig:kkl_ae}.
To train this model, a grid of $N$ datapoints $x_i$ is generated with LHS or any other method, then the weights $\param$ and $\invparam$ are optimized using gradient-based methods to minimize~\eqref{eq:optimization_jointly}. Autoencoders 

\subsection{Optimizing D jointly}
\label{subsec:optimizing_D_jointly}

One of the main advantages of the AE model in Fig.~\ref{fig:kkl_ae} is that it enables the user to optimize $D$ jointly with the network weights.
This has already been implemented in the context of nonlinear system identification in~\citet{Andrieu_deepKKL_output_prediction_nonlin_systs} for example.
It can be done naturally by adding $D$ to the model parameters when minimizing~\eqref{eq:optimization_jointly}.

We train the AE in the same settings as the previous experiments on the reverse Duffing oscillator~\eqref{eq:rev_duffing} with $\lambda=0.1$ and $N=70,000$. We initialize $D$ as~\eqref{eq:D} with $\omegac = 0.2$. After training, $D$ has almost the same eigenvalues as at the initialization, and we observe similar performance to the previous supervised method, as illustrated in Fig.~\ref{fig:rev_duffing_test_trajs_AE}.
Initializing with $\omegac=0.5$ slightly deteriorates the performance (RMSE = 0.12 on the test trajectory in Fig.~\ref{fig:rev_duffing_test_trajs_AE}) while the eigenvalues of $D$ slightly decrease during training; they slightly increase when initializing with $\omegac=0.1$ (RMSE = 0.1).
These experiments demonstrate that it is possible to learn KKL observers by training an autoencoder from samples in $\X$ only, and to optimize the tuning parameters jointly with the model weights. With this unsupervised method also, initializing $D$ as~\eqref{eq:D} with $\omegac \approx 0.2$ yields good performance in the presence of noise.

From then on, it is possible to add other terms to~\eqref{eq:optimization_jointly} to penalize other aspects, e.g., noise sensitivity, by adding our gain tuning criterion~\eqref{eq:gain_tuning_criterion} which depends both on $\param$ and on $D$ to the loss. This could be a good direction for future research, but requires significant implementation efforts to implement cost functions resembling \eqref{eq:gain_tuning_criterion} in automatic differentiation software.

% This approach has already been implemented in the context of nonlinear system identification in~\citet{Andrieu_deepKKL_output_prediction_nonlin_systs} and we leave its implementation for observer design as future work. 



\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.9\columnwidth]{figures/revduffing_ae_portrait_wc02.pdf}
		\setlength{\belowcaptionskip}{-10pt}
        \setlength{\abovecaptionskip}{-2pt}
		\caption{Estimated trajectory of the reverse Duffing oscillator starting at $x(0)=(0.6,0.6)$ using an autoencoder and optimizing $D$ jointly with the model weights. $D$ is initialized as~\eqref{eq:D} with $\omegac = 0.2$, and the measurement is corrupted by Gaussian noise $\mathcal{N}(0, 0.5)$ as in the bottom line of  Fig.~\ref{fig:rev_duffing_test_trajs}.}
		\label{fig:rev_duffing_test_trajs_AE}
	\end{center}
\end{figure}

